A framework for window design in delivery schedules

This paper develops a structured framework for the design and dynamic updating of service time windows in delivery and appointment-based systems. We consider a single-server setting with stochastic service and travel times, where customers are promised a time window in which the provider will arrive. The first part of the paper introduces a static window construction method based on a probabilistic threshold criterion, using an analytical approximation of residual travel and service time distributions. Building on this, we develop a dynamic update mechanism that monitors residual system uncertainty, where time windows are revised during execution only when the remaining time until the window's start falls below a predefined threshold. This threshold-based approach enables communication-efficient scheduling while substantially improving delivery accuracy. Numerical experiments demonstrate significant performance gains of the dynamic approach in both stylized and real-world settings.

==> Sections/Analysis.tex <==
\iffalse
\section{Analysis}
Note that the problem ${\rm WOS}_n({\bs B},\omega,f)$ fully decouples: there are $n$ independent optimization problems, where the objective function of the $i$-th is
\[H_i(t_i,\Delta_i):=\omega  {\mathbb E}\left(S_i-t_i-\Delta_i\right)^+
+(1-\omega){\mathbb E}\left(t_i-S_i\right)^+ + f(\Delta_i).\]
Observe the strong similarity to the classical {\it news vendor problem}. The optimization can be analyzed by evaluating the first order conditions:
\[\frac{\partial H_i(t_i,\Delta_i)}{\partial t_i} = -\omega (1-F_i(t_i+\Delta_i)) +(1-\omega)F_i(t_i)=0,\]
and
\[\frac{\partial H_i(t_i,\Delta_i)}{\partial \Delta_i} = -\omega (1-F_i(t_i+\Delta_i)) +f'(\Delta_i)=0.\]
Let us first focus on the partial derivative with respect to $t_i$. Considering, for a given value of $\Delta_i$ the equation
\[\omega (1-F_i(t_i+\Delta_i)) =(1-\omega)F_i(t_i),\]
we can argue there is a unique solution for continuous distribution functions $F_i(\cdot)$.
Observe that the left-hand side has the value $\omega(1-F_i(\Delta_i))\geqslant 0$ at $t_i=0$, and decreases to $0$ as $t_i\to\infty$. At the same time, the right-hand side has the value $0$ at $t_i=0$, and increases to $(1-\omega)$ as as $t_i\to\infty$. We denote the intersection point by $t_i(\Delta_i)$. It is directly verified from the fact that $\omega(1-F_i(\Delta_i))$ decreases in $\Delta_i$ that $t_i(\Delta_i)$ decreases in $\Delta_i$ as well. 

From the partial derivative with respect to $\Delta_i$, we can determine the sole remaining unknown $\Delta_i$ from the equation
\[\omega (1-F_i(t_i(\Delta_i)+\Delta_i)) =f'(\Delta_i).\]
\textcolor{red}{Why should such a solution exist?}
My hunch is that for some forms of the penalty function $f(\cdot)$ one could get $\Delta =0$ (when you have a very steep $f(\cdot)$) or $\Delta = \infty$ (when you have a very flat $f(\cdot)$). 

\textcolor{red}{Equating the rhs of
the equations above, we find that,
whenever the inverse of the distribution
function of $S_i$ exists and whenever
$f'(\Delta_i) \in [0,1-\omega]$,
\begin{align*}
    t_i &= F_i^{-1}\left(
    \frac{f'(\Delta_i)}{1-\omega}
    \right).
\end{align*}
Inserting this in the second
equation and rearranging terms,
we obtain that
whenever $f'(\Delta_i) \in [0,\omega]$,
\begin{align*}
    \Delta_i &= 
    F_i^{-1}\left(1-
    \frac{f'(\Delta_i)}{\omega}
    \right)
    -
    F_i^{-1}\left(
    \frac{f'(\Delta_i)}{1-\omega}
    \right).
\end{align*}
Thus, if we find a $\Delta_i$ for which
$f'(\Delta_i) \in [0,\min\{\omega, 1-\omega\}]$ and which satisfies the
equation above, we can solve for the optimal
$(t_i,\Delta_i)$ in case the solution yields both $t_i \geq 0$ and $\Delta_i \geq 0$. That is, we must have
\begin{align*}
    F_i^{-1}\left(
    \frac{f'(\Delta_i)}{1-\omega}
    \right) \geq 0 \qquad \text{and}
    \qquad 
    F_i^{-1}\left(1-
    \frac{f'(\Delta_i)}{\omega}
    \right)
    -
    F_i^{-1}\left(
    \frac{f'(\Delta_i)}{1-\omega}
    \right) \geq 0,
\end{align*}
or, equivalently,
\begin{align*}
    F_i^{-1}\left(
    \frac{f'(\Delta_i)}{1-\omega}
    \right) \geq 0 \qquad \text{and}
    \qquad 
    \omega(1-\omega) \geq f'(\Delta_i).
\end{align*}
}


\vb

The problem ${\rm UWOS}_n({\bs B},\omega,f)$ evidently does not decouple, but the above approach by and large carries over. We obtain that the optimizing $t_i$ are of the form $t_i(\Delta)$ as defined above, where $\Delta$ solves
\[\omega \sum_{i=1}^n  (1-F_i(t_i(\Delta)+\Delta))= nf'(\Delta).\]

The distribution function $F_i(\cdot)$ can be evaluated efficiently using standard ideas for numerical convolutions that we investigated in the context of Paper 1. See the earlier document by Roshan; this we can actually put into an appendix. When discretizing, the function $t_i(\cdot)$ may be a bit harder to get, so we have to think about that. 

\textcolor{red}{\textbf{Analysis for the general objective function} 
\begin{align*}
    G_n({\bs t},{\bs \Delta}):= \omega\sum_{i=1}^n {\mathbb E}\left(\left(S_i-t_i-\Delta_i\right)^+\right)^{m_i}
+(1-\omega)\sum_{i=1}^n {\mathbb E}\left(\left(t_i-S_i\right)^+\right)^{\ell_i} +\sum_{i=1}^n f(\Delta_i).
\end{align*}
We have
\begin{equation*}
H_i(t_i, \Delta_i) = \omega \mathbb{E}\left(\left(\left(S_i - t_i - \Delta_i\right)^+\right)^{m_i}\right) + (1-\omega) \mathbb{E}\left(\left(\left(t_i - S_i\right)^+\right)^{\ell_i}\right) + \sum_{i=1}^n f(\Delta_i).
\end{equation*}
\begin{align*}
   \omega\mathbb{E}\left(\left(S_i - t_i - \Delta_i\right)^+\right)^{m_i} + (1-\omega)\mathbb{E}\left(\left(t_i - S_i\right)^+\right)^{\ell_i}
   &= \omega \int_{t_i+\Delta_i}^\infty (x - t_i - \Delta_i)^{m_i} f_i(x) \, dx \\& + (1-\omega) \int_{0}^{t_i} (t_i - x)^{\ell_i} f_i(x) \, dx
\end{align*}
\begin{equation*}
     \frac{\partial H_i(t_i,\Delta_i)}{\partial t_i} = -m_i \omega\int_{t_i+\Delta_i}^\infty (x - t_i - \Delta_i)^{m_i-1} dF_i(x) +(1-\omega)\ell_i \int_{0}^{t_i} (t_i - x)^{\ell_i-1} dF_i(x)
\end{equation*}
and
\begin{equation*}
     \frac{\partial H_i(t_i,\Delta_i)}{\Delta_i} = -m_i \omega\int_{t_i+\Delta_i}^\infty (x - t_i - \Delta_i)^{m_i-1} dF_i(x) +f'(\Delta_i)
\end{equation*}
Assume all integrals to converge. Then,
with a similar reasoning as above, we can argue
that when equating the first partial derivative
to zero, we are able to find a solution $t_i(\Delta_i)$. Note, however, that uniqueness
is no longer guaranteed. Equating the second
partial derivative to zero then yields the unknown
$\Delta_i$ (that is, if a solution to this equation exists).
}

\begin{remark}
    If solutions to the equations above exist, we may be able
    to handle polynomial objective functions. However, it seems that we are not able to handle functions like
    \begin{equation*}
H_i(t_i, \Delta_i) = \omega \mathbb{E}\left(\text{arctan}\left(\left(S_i - t_i - \Delta_i\right)^+\right)\right) + (1-\omega) \mathbb{E}\left(\text{arctan}\left(\left(t_i - S_i\right)^+\right)\right) + \sum_{i=1}^n f(\Delta_i),
\end{equation*}
as we obtain
\[\frac{\partial H_i(t_i,\Delta_i)}{\partial t_i} = -\omega 
\int_{t_i + \Delta_i}^\infty \frac{1}{1 + (x-t_i-\Delta_i)^2} f_i(x)dx
+ (1-\omega) 
\int_0^{t_i} \frac{1}{1 + (t_i-x)^2} f_i(x)dx
=0,\]
and
\[\frac{\partial H_i(t_i,\Delta_i)}{\partial \Delta_i} = -\omega 
\int_{t_i + \Delta_i}^\infty \frac{1}{1 + (x-t_i-\Delta_i)^2} f_i(x)dx +f'(\Delta_i)=0,\]
but if we require 
\[\omega 
\int_{t_i + \Delta_i}^\infty \frac{1}{1 + (x-t_i-\Delta_i)^2} f_i(x)dx
= (1-\omega) 
\int_0^{t_i} \frac{1}{1 + (t_i-x)^2} f_i(x)dx,\]
we note that the lhs starts at a non-negative value and, as $t_i \to \infty$,
goes to 0. However, whereas the rhs for $t_i = 0$ equals 0, we 
also have that its limit in $t_i$ approaches 0 (for some
forms of $f(x)$, such as $f(x) = e^{-x}$). Therefore,
a solution to this equation is not guaranteed to exist. It seems that in general,
for $g, h: \mathbb{R} \to \mathbb{R}$
and
  \begin{equation*}
H_i(t_i, \Delta_i) = \omega \mathbb{E}\left(g\left(\left(S_i - t_i - \Delta_i\right)^+\right)\right) + (1-\omega) \mathbb{E}\left(h\left(\left(t_i - S_i\right)^+\right)\right) + \sum_{i=1}^n f(\Delta_i),
\end{equation*}
a value for $t_i(\Delta_i)$ can be found
if (but definitely not only if), for $t > 0$,
$g'(t) > 0$,
$h'(t) \geq 0$, and $\lim_{t \to \infty}h'(t)f_i(t) \neq 0$.
\end{remark}
\fi


\iffalse
\section{Experiments}
     One interesting experiment: how much do you lose when taking the $\Delta_i=\Delta$ for each $i$?

Notes for the implementation:
\begin{itemize}
    \item[$\circ$] Solving the equations in the WOS-setting is trivial (i.e., when one has access to a numerical solver) in the case $F_i(\cdot)$ is known.
    \item[$\circ$] One natural way to find $F(\cdot)$ is to start with distributions
    $G_i(\cdot)$ for each $B_i$ in the discretized pdf form
    $\{(t_{i,1}, p_{i,1}), (t_{i,2}, p_{i,2}), \dots\}$, where
    $p_{i,j}$ is the probability that the
    discretized version of $B_i$ takes the
    value $t_{i,j}$.
    The distribution of $B_1 + B_2$ is now
    simply given by all pairs $(t, p)$, where
    $t = t_{1,k} + t_{2,l}$ and
    $p = p_{1,k} + p_{2,l}$ for some $k,l > 0$.
    We can then iteratively continue to find the distribution of $B_1 + B_2 + B_3$, by
    combining the list of $B_1 + B_2$, and the 
    given discretized pdf of $B_3$.
    \end{itemize}

One could try to study more systematically the impact of the shape of the penalty function on the windows. 
  \begin{itemize} 
  \item[$\circ$] We take ${\mathscr P}(\Delta) = (\alpha/\beta) \Delta^\beta$, and include figures
  (Figures~\ref{fig:exp1_v1} and~\ref{fig:exp1_v2}) of $(t_i,t_i+\Delta_i)$ as functions of $i$ for $\alpha$ fixed and different values of $\beta\in[1,2)$.
  The following observations can be made:
  \begin{itemize}
      \item Impact of $\omega$:
      \item Impact of $b$:
      \item Impact of $\alpha$:
      \item Interesting observation from Figure~\ref{fig:exp1_v2}:
  \end{itemize}
    \item[$\circ$] In the case that we work with the penalty function ${\mathscr P}(\Delta) = (\alpha/\beta) \Delta^\beta$ and $B_i \sim N(\mu,\sigma^2)$, we try to fit functions
    $\varphi(\cdot)$ and $\psi(\cdot)$ such that
    \[\varphi(i) \approx t_i,\:\:\:\psi(i)\approx \Delta_i.\]
    Without loss of generality we can assume that $\mu\equiv 1$ (this is just a time rescaling), so  $\varphi(\cdot)$ and $\psi(\cdot)$ are functions of $\sigma,$ $\alpha$, $\beta$, $\omega$. One case we know explicitly, viz.\ the one with $\beta = 1$. For general $\beta \in [1,2)$, we fit a power law 
    to $\varphi(i)-i$ and to $\varphi(i)+\psi(i)-i$. A few of the fits (obtained via the `curve fit' method in Python) are presented in Figures~\ref{fig:power_law_fit_v1},
    \ref{fig:power_law_fit_v2a}
    \ref{fig:power_law_fit_v3}, and \ref{fig:power_law_fit_v2}. Note that, whereas some fits seem extremely well, there are also cases for which the fits seem less appropriate. Unfortunately, no pattern has been discovered yet. 
    \end{itemize}
\fi

\iffalse
\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{Figures/ti_windowi_matrix_plot_v1.pdf}
    \caption{Normal distribution, parameters $\mu_i = 2.0$ and $\sigma_i = 0.1$.}
    \label{fig:exp1_v1}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{Figures/ti_windowi_weibull.pdf}
    \caption{Weibull distribution, parameters $\mu_i = 2.0$ and $\sigma_i = 0.1$.}
    \label{fig:exp1_weibull}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{Figures/ti_windowi_lognormal.pdf}
    \caption{Lognormal distribution, parameters $\mu_i = 2.0$ and $\sigma_i = 0.1$.}
    \label{fig:exp1_lognormal}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{Figures/ti_windowi_matrix_plot_v2.pdf}
    \caption{Normal distribution, parameters $\mu_i = 15.0$ and $\sigma_i = 1.0$.}
    \label{fig:exp1_v2}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{Figures/ti_windowi_weibull_v2.pdf}
    \caption{Weibull distribution, parameters $\mu_i = 15.0$ and $\sigma_i = 1.0$.}
    \label{fig:exp1_v2_weibull}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{Figures/ti_window_lognormal_v2.pdf}
    \caption{Lognormal distribution, parameters $\mu_i = 15.0$ and $\sigma_i = 1.0$.}
    \label{fig:exp1_v2_lognormal}
\end{figure}
\fi

==> Sections/Dynamic_Procedure.tex <==
\section{Dynamic procedure}\label{sec:dyn}



In this section we study the dynamic procedures that have been proposed in Section~\ref{subsec:dyn}. 
In the computations presented below we work in the setting that all travel times are independent normally distributed random variables, which we have shown to be an accurate proxy in Section~\ref{subsec:WOSnorm}, but in principle one could also work with generally distributed travel times using the machinery of Section~\ref{subsec:WOSgen}.


\begin{algorithm}[ht]
 \KwResult{Time window}
 a. Initialization: set $F_i = 0$
 for $i = 1,\dots,n$, $N_0 = 1$
 and $b_0 = 0$\;
 b. Let $(\boldsymbol{\tau},
 \boldsymbol{\Delta})$ be a minimizer
 of WOS$_n$($\boldsymbol{B}, \omega,
 \mathcal{P}$)
 c. \For{$j = 1,\dots$}{
    1. Update $N_j$ and $b_j$ 
    2. Let $(\boldsymbol{\tau},
 \boldsymbol{\Delta})$ be a minimizer
 of WOS$_n$($\boldsymbol{B}, \omega,
 \mathcal{P}$)\;
    3. \For{$i = N_j,\dots,n$}{
    If $t_i - \tau \cdot j \leq T$
    and $F_i = 0$:
    communicate $(t_i, t_i + \Delta_i)$
    }
    }
 \caption{Optimal departure time online setting.}
  \label{alg:online}
\end{algorithm}




% \subsection{Rolling horizon updates}
% The third flavor involves a rolling-horizon approach, where we dynamically determine when to provide time-window updates. Our goal is to develop an approach that works well in real-world settings. 
% Let $\tau$ be the time between potential updates. For client $i$, denote by $t_i^j$ and $\Delta_i^j$ the start time and width of the time window, respectively, at the $j$-th potential update instant, i.e., at time $j\tau$. 
% To control the number of updates, the objective needs to incorporate the dissatisfaction of clients resulting from time-window updates. 
% We adopt a similar framework as in \cite{DSW}, expressing client dissatisfaction as the sum of two components, $g$ and $h$. The function $g$ accounts for dissatisfaction arising from time-window updates, while $h$ captures the quality of the final announced time window, as in Section~\ref{sec:framework}. 
% More specifically, define the dissatisfaction of client $i$ for time-window updates at time $j \tau$ as 
% \begin{align*}
%     g_{i,j}(t_i^{j-1}, \Delta_i^{j-1}, t_i^{j}, \Delta_i^{j}) 
%     \; = \;\; &
%     w_1 f_j(t_i^j) \left(t_i^{j-1}- t_i^{j}\right)^+ + w_2 \left(t_i^{j}+ \Delta_i^{j} - t_i^{j-1}- \Delta_i^{j-1}\right)^+  \\  
%     \;\; & + \; w_3 \;  \mathbf{1}_{\left\{\left(t_i^j, \Delta_i^j\right) \neq 
%     \left(t_i^{j-1}, \Delta_i^{j-1}\right)\right\}},
%     %+ w_4(t_i^{j}-t_i^{j-1}<\theta)
% \end{align*}
% for some parameters $w_1, w_2, w_3 \ge 0$ and function $f_j(\cdot)$. 
% To make updates rewarding, we assume that $w_1 < 1-w$ and $w_2 < w$.
% The first two terms of $g_{i,j}(\cdot)$ represent dissatisfaction due to shifting the start of the time window earlier and extending its end, respectively. The third term captures a fixed penalty for any change to the time window. 
% We adopt the function proposed in \cite{DSW} to capture the effect of the adjustment's proximity to the start of the time window:
% \begin{equation*}
%     f_j(t_i) = 1 + \nu \left( j \tau - (t_i - L) \right)^+,
% \end{equation*}
% for non-negative parameters $\nu$ and $L$.
% If the adjustment is announced at least $L$ time units before the new start time, i.e., $t_i - j \tau \geq L$, then $f_j(t_i) = 1$, meaning no additional dissatisfaction is incurred. However, adjustments communicated within $L$ time units of the new start are penalized at a linear rate $\nu$.
% \newline
% The rolling horizon approach works as follows. Initially, each client is assigned a time window based on the WOS. Specifically, for client~$i$, the initial time-window parameters $t_i^0$ and $\Delta_i^0$ are determined by
% \[
% (t_i^0, \Delta_i^0) = \arg\min_{t,\, \Delta \ge 0} H_i(t, \Delta).
% \]
% Now, at the $j$-th potential update epoch, a new window is communicated if the improvement exceeds the dissatisfaction due to updating. Note that the latest communicated window before $j \tau$ yields objective $H_{i,j}'(t_i^{j-1}, \Delta_i^{j-1})$. Using DWOS-T, a potential new time window provides objective 
% \[ 
% (\tilde t, \tilde \Delta) = \arg\min_{t,\, \Delta \ge 0} H_{i,j}'(t, \Delta).
% \]
% New time-window parameters $(t_i^j, \Delta_i^j) = (\tilde{t}, \tilde{\Delta})$ are communicated to client~$i$, provided the client still requires service, if
% \[
% g_{i,j}(t_i^{j-1}, \Delta_i^{j-1}, \tilde{t}, \tilde{\Delta}) + H_{i,j}'(\tilde{t}, \tilde{\Delta}) < H_{i,j}'(t_i^{j-1}, \Delta_i^{j-1}).
% \]
% Otherwise, the previous window is retained, that is, $t_i^j = t_i^{j-1}$ and $\Delta_i^j = \Delta_i^{j-1}$.
% \newline
% We utilize DWOS-T at each step in the rolling-horizon approach, which ensures that the rolling-horizon approach remains tractable. Moreover, the method readily accommodates alternative choices for the dissatisfaction function~$g$ without compromising computational performance. Its intuitive update logic further supports its suitability for practical implementation.
% \newline
% For communicated sequences of time-window parameters $(\bs t, \bs \Delta)$, the dissatisfaction is then implicitly defined as
% \begin{align*}
%    \mbox{\rm DWOS-R}_n({\bs B},\omega,{\mathscr P},\tau, \bs t, \bs \Delta):= \sum_{i=1}^n g_i(\bs t_i, \bs \Delta_i) + h_i(\bs t_i, \bs \Delta_i), 
% \end{align*}
% with 
% \begin{align*}
%     g_i(\bs t_i, \bs \Delta_i) & \; = \;  \sum_{j=0}^\infty 
%     g_{i,j}(t_i^{j-1}, \Delta_i^{j-1}, t_i^{j}, \Delta_i^{j}) \\
%     h_i(\bs t_i, \bs \Delta_i) & \; = \; 
%     \mathbb{E} \left[ \sum_{j = 0}^{\infty}
%     \left(
%     \omega \left(S_i - t_i^j\right)^+ +
%     (1-\omega) \left(t_i^j + \Delta_i^j -S_i\right)^+
%     + {\mathscr P}(\Delta_i^j) \right)
%     \mathbf{1}_{j\tau < S_i \le (j+1)\tau} \right].
% \end{align*}


% \Rene{
% THIS IS WRITTEN FOR OURSELVES
% \newline
% For each client $i$, we can compare the performance based on the following four performance measures:
% \begin{itemize}
%     \item Total objective value: $g_i(\bs t_i, \bs \Delta_i) + h_i(\bs t_i, \bs \Delta_i)$
%     \item Quality of final time window: $h_i(\bs t_i, \bs \Delta_i)$
%     \item Dissatisfaction from updates: $g_i(\bs t_i, \bs \Delta_i)$
%     \item Number of (communicated) updates
% \end{itemize}
% Initially, we should this for all clients $i$ to get a feeling for the trade-off between frequency of updating and improvement. Of course, we can also do this by summing over all clients.
% Also, we can `play' a bit with the parameters, as we have quite some: $w_1, w_2, w_3, \nu, L$. 
% \newline
% To `benchmark' our results, I think we should compute $g_i(\bs t_i, \bs \Delta_i)$ as well for \emph{index-triggered} and \emph{time-triggered} updates. The case $N=1$ for the index-triggered updates should provide a kind of lower bound for the $h_i(\bs t_i, \bs \Delta_i)$ part of the objective for the rolling-horizon approach.
% }

% \subsection{Dalmeijer equivalent}
% Let $\tau$ be the length of time after we
% update, and $\bs t$ and $\bs \Delta$
% are the communicated starting times and
% windows widths.
% For each customer~$i$, the penalty function is G.
% \begin{align*}
%     \sum_{j = 0}^\infty 
%     g_{i,j}(t_i^{j-1}, \Delta_i^{j-1}, t_i^{j}, \Delta_i^{j}) 
%     + 
%     h_i(\bs t, \bs \Delta)
% \end{align*}
% where $G= \sum_{j = 0}^\infty 
%     g_{i,j}(t_i^{j-1}, \Delta_i^{j-1}, t_i^{j}, \Delta_i^{j}) $
% \begin{align*}
%     h_i(\bs t, \bs \Delta) = 
%     \sum_{j = 0}^{\infty}
%     \left(
%     \omega \left(S_i - t_i^j\right)^+ +
%     (1-\omega) \left(t_i^j + \Delta_i^j -S_i\right)^+
%     \right)
%     1_{j\tau < S_i}
%     1_{(j+1)\tau > S_i}
% \end{align*}
% and
% \begin{align*}
%     g_{i,j}(t_i^{j-1}, \Delta_i^{j-1}, t_i^{j}, \Delta_i^{j}) 
%     &=
%     w_1^j(t_i^{j-1}- t_i^{j})^+ + w_2^j \left((t_i^{j}+ \Delta_i^{j} - t_i^{j-1}- \Delta_i^{j-1})\right)^+ \\
%     & \qquad + w_3 1_{(t_i^j, \Delta_i^j) \neq 
%     (t_i^{j-1}, \Delta_i^{j-1})}
%     %+ w_4(t_i^{j}-t_i^{j-1}<\theta)
%     + P_{i,j}(\Delta_i^j) 
% \end{align*}

% Heuristics:
% \begin{itemize}
%     \item Algorithm 1
%     \item Algorithm 2
%     \item $\cdots$
% \end{itemize}

% Let $(t_i^0, \Delta_i^0)$ be initial time window; $(t_i^j, \Delta_i^j)$ be the internally updated window at every $j\tau$; $(\hat{t_i}^j, \hat{\Delta_i}^j)$ be the last communicated window to the client; $U_i$ count of updates communicated to client i; say $K$ is the cap/threshold  for $U_i$ as we don't to communicate more than perhaps 5-6 times and a threshold $\zeta$ on penalty function such that if the changes in TW aren't major we do not notify the clients. 

% \begin{enumerate}
%     \item evaluate initial TW initial time windows $(t_i^0, \Delta_i^0)$ for all $i=1,\dots,n$
%     \item for each update epoch update epoch $T = j\tau$; set $(\hat{t_i}^j, \hat{\Delta_i}^j)\leftarrow (t_i^0, \Delta_i^0)$ and $U_i\leftarrow 0$
%     \begin{itemize}
%         \item use the procedure of algo-2 to evaluate $(t_i^j, \Delta_i^j)$
%         \item evaluate the penalty  $\sum_{j = 0}^\infty 
%     g_{i,j}(t_i^{j-1}, \Delta_i^{j-1}, t_i^{j}, \Delta_i^{j}) $
%     \item if $g_{i,j}>\zeta$ or $U_i>K$ then do not communicate
%     \item else: update $\hat{t_i}^j\leftarrow t_i^j$ and  $\hat{\Delta_i}^j\leftarrow \Delta_i^j$, $U_i+=1$
%     \end{itemize}
% \end{enumerate}

==> Sections/StaticWOS.tex <==
\section{Optimal windows: the static WOS case}\label{sec:wos}
In this section we present our analysis of the static WOS case. In Section \ref{subsec:foc} we present the underlying first order conditions, and show that under mild conditions they have a unique solution. As it turns out, in case the service times $B_i$, $i=1,\ldots,n$, stem from a normal distribution, a fairly explicit analysis can be performed; see Section \ref{subsec:WOSnorm}. The case with generally distributed service times is addressed in Section \ref{subsec:WOSgen}.  

\subsection{First-order conditions} \label{subsec:foc}
We start by presenting the first-order conditions pertaining to the optimization problem 
${\rm WOS}_n({\bs B},\omega,\mathscr{P})$. Using standard differentiation rules, it is readily verified that these read
\begin{align}
    \frac{\partial}{\partial t_i} G_n({\bs t},{\bs \Delta}) &=  (1-\omega)F_i(t_i)- \omega(1-F_i(t_i + \Delta_i))=0 ,\label{FOC1}\\
    \frac{\partial}{\partial \Delta_i} G_n({\bs t},{\bs \Delta}) &= - \omega(1-F_i(t_i + \Delta_i)) + {\mathscr P}'(\Delta_i)=0 \label{FOC2}.
\end{align}
As mentioned above, the $2n$-dimensional optimization problem decouples into $n$ individual two-dimensional optimization problems that can be solved separately. This means that, in this static WOS setting, determining the optimal window assignment is of low computational complexity. 


To gain some intuition about the nature of the solution of Equations \eqref{FOC1}--\eqref{FOC2}, we consider the specific case of a linear cost function:
${\mathscr P}(\Delta) = \alpha \Delta$. 
For any general underlying service-time distribution and $\omega \in (0,1)$
we can obtain the corresponding result.
That is, combining the first two equations yields
\begin{align*}
    (1-\omega)F_i(t_i) = \alpha,
\end{align*}
from which we obtain that we should have $\alpha \leqslant 1 - \omega$ to have a stationary point. The second equation yields
\begin{align*}
    \omega(1-F_i(t_i + \Delta_i)) = \alpha,
\end{align*}
which only has a solution if $\alpha \leqslant \omega$. Therefore, only in the case
$\alpha \leqslant \min\{\omega, 1-\omega\}$ one has that the
optimum corresponds to a stationary point of the objective function (which implies that we should necessarily have $\alpha\leqslant \frac{1}{2}$).
Moreover, it is trivially seen that when
the inverse of the distribution function of
$S_i$ exists, one has
\begin{align*}
    t_i &= F_i^{-1}\left(\frac{\alpha}{1-\omega}\right),\quad
    \Delta_i = F_i^{-1}\left(1-\frac{\alpha}{\omega}\right) - F_i^{-1}\left(\frac{\alpha}{1-\omega}\right),
\end{align*}
in other words, the window starts at $F_i^{-1}(\frac{\alpha}{1-\omega})$ and ends at $F_i^{-1}(1-\frac{\alpha}{\omega})$. 


The fact that we only get a non-degenerate result for $\alpha \leqslant \min\{\omega, 1-\omega\}$ is a consequence of the linear window cost: if ${\mathscr P}(\cdot)$ is proportional to a constant $\alpha$, then ${\mathscr P}'(\Delta)$ equals this $\alpha$, thus rendering solving the two first-order conditions simultaneously problematic. This complication does not play any role when picking, for instance, ${\mathscr P}(\Delta) = (\alpha/\beta) \Delta^\beta$, with $\alpha > 0$, $\beta>1$. 
The following theorem provides sufficient conditions under which the optimal $\Delta_i$ and $t_i$ can be uniquely found from the first-order conditions. 

\begin{theorem}\label{THM1}
Let ${\mathscr P}(\cdot)$ be strictly convex, and let $g(\Delta):={\mathscr P}'(\Delta)$ have a continuous inverse. Then \eqref{FOC1} and \eqref{FOC2} have a unique positive solution for $(t_i,\Delta_i)\in{\mathbb R}_+^2$,
\nac{which yields the minimum ${\rm WOS}_n({\bs B},\omega,\mathscr{P})$.}
\end{theorem}

{\it Proof.}
 Realize that $g(\Delta):={\mathscr P}'(\Delta)$ is increasing in $\Delta$, and assume that $g(\cdot)$ is invertible. Hence,
\[\Delta_i(t_i) = g^{-1}((1-\omega)F_i(t_i)),\]
which is increasing in $t_i$ (as it is the composition of the increasing functions $g^{-1}(\cdot)$ and $F_i(\cdot)$).
We thus obtain the equation
\[{\mathfrak f}^-_i(t_i):= \omega\left(1-F_i\left(t_i +g^{-1}((1-\omega)F_i(t_i)\right)\right) = (1-\omega)F_i(t_i) =:{\mathfrak f}^+_i(t_i).  \]
Observe that ${\mathfrak f}^-_i(\cdot)$ is decreasing, with ${\mathfrak f}^-_i(0)= \omega$ and ${\mathfrak f}^-_i(\infty)=0$, and that ${\mathfrak f}^+_i(\cdot)$ is increasing, with ${\mathfrak f}^+_i(0)= 0$ and ${\mathfrak f}^+_i(\infty)=1-\omega.$ Conclude that there is a unique positive root for any $\omega\in(0,1).$ 

To verify whether the found stationary point is indeed a {\it minimum}, we consider the Hessian, using the familiar notation $f_i(t):=F_i'(t)$,
\[ \left(\begin{array}{cc}(1-\omega)f_i(t_i)+\omega f_i(t_i+\Delta_i)&\omega f_i(t_i+\Delta_i)\\
\omega f_i(t_i+\Delta_i)
&\omega f_i(t_i+\Delta_i)+{\mathscr P}''(\Delta_i)\end{array}\right).\]
This matrix is diagonally-dominant, hence positive definite (where it is used that ${\mathscr P}(\cdot)$ being strictly convex entails ${\mathscr P}''(\Delta_i)>0$). It follows that it has positive eigenvalues, which implies that any stationary point (i.e., solution of the first-order conditions) is a minimum.
\hfill$\Box$


For instance, in the case of ${\mathscr P}(\Delta) = (\alpha/\beta) \Delta^\beta$ we obtain the first-order conditions
\[ (1-\omega)F_i(t_i) = \alpha\,\Delta_i^{\beta-1}, \quad \omega(1-F_i(t_i + \Delta_i)) = \alpha \,\Delta_i^{\beta-1}.\]
Solving $\Delta_i$ from the first of these two equations, we find
\[\Delta_i(t_i) = \left(\frac{1-\omega}{\alpha}F_i(t_i)\right)^{1/(\beta-1)},\]
which is an increasing function of $t_i$. Then $t_i$ is found from the equation ${\mathfrak f}^-_i(t_i)={\mathfrak f}^+_i(t_i)$.

% \begin{remark}{\em 
% \Rene{Or incorporate in Theorem \ref{THM1}??}
% Theorem \ref{THM1} gives conditions under which there is a unique stationary point for $(t_i,\Delta_i)\in{\mathbb R}_+^2.$
% To verify whether the found stationary point is indeed a {\it minimum}, we consider the Hessian, using the familiar notation $f_i(t):=F_i'(t)$,
% \[ \left(\begin{array}{cc}(1-\omega)f_i(t_i)+\omega f_i(t_i+\Delta_i)&\omega f_i(t_i+\Delta_i)\\
% \omega f_i(t_i+\Delta_i)
% &\omega f_i(t_i+\Delta_i)+{\mathscr P}''(\Delta_i)\end{array}\right).\]
% This matrix is diagonally-dominant, hence positive definite (where it is used that ${\mathscr P}(\cdot)$ being strictly convex entails ${\mathscr P}''(\Delta_i)>0$). It follows that it has positive eigenvalues, which implies that any stationary point (i.e., solution of the first-order conditions) is a minimum. }
% \hfill$\Diamond$
% \end{remark}





%\begin{definition}[Exogenous-endogenous schedule] For a given $n\in{\mathbb N}$, random vector ${\bs B}\in {\mathbb R}^n_+$, weight $\omega \in (0,1)$, and increasing penalty function $f:{\mathbb R}_+\to {\mathbb R}_+$, and exogenous time windows
%$[s_i, e_i]$, define
%\[{\rm EEOS}_n({\bs B},\omega,f,{\bs e},{\bs s}):= \min_{{\bs t}\in {\mathbb R}_+^d,{\Delta}\in{\mathbb R}_+: 
%s_i \leq t_i \leq t_i + \Delta_i \leq e_i}G_n({\bs t},\Delta).\]
%\end{definition}

\subsection{WOS under the normal distribution}\label{subsec:WOSnorm}
In the above, the travel times $B_i$ are defined in a general form. 
Here, we investigate the specific case that the travel time distributions
are independent random variables with a normal distribution,
as, in that case, the distribution of $S_i$ is
normally distributed as well. 

Let $B_i \sim N(\mu_i,\sigma_i^2)$, 
with $B_1,B_2,\dots$ independent, and with $\mu_i>0$ and $\sigma_i\ll \mu_i$. The requirement $\sigma_i\ll \mu_i$ is intended to make sure that the probability mass on the negative numbers is effectively negligible; in practical terms $\sigma_i < \mu_i/3$ suffices, as this yields a probability of a negative travel time of just over $10^{-3}$. Considering the problem
${\rm WOS}_n({\bs B},\omega,{\mathscr P})$, the crucial observation is  that
$S_i\sim N(\tilde\mu_i,\tilde\sigma_i^2)$ with $\tilde{\mu}_i := \sum_{j = 1}^i \mu_j$ and 
$\tilde{\sigma}_i^2 := \sum_{j = 1}^i \sigma_j^2$, i.e.,
\begin{align*}
    F_i(t) = \Phi\left(\frac{t-\tilde{\mu}_i}{\tilde{\sigma}_i} \right),
\end{align*}
with $\Phi(\cdot)$ the cumulative distribution function of a standard normal random variable. 
From \eqref{FOC1} and \eqref{FOC2}, it follows that we are to solve the equations
% Consider the original objective function $G_n({\bs t},{\bs \Delta})$ (i.e., the one of Remark \ref{R1} with $\ell_i=m_i=1$), and take the partial derivative with respect to $t_i$ and $\Delta_i$.
% Performing this calculation, it turns out that we are to solve the equations
\begin{align*}
    \omega\left(1-\Phi\left(\frac{t_i+\Delta_i-\tilde{\mu}_i}{\tilde{\sigma}_i} \right)\right)
    &= (1-\omega)\Phi\left(\frac{t_i-\tilde{\mu}_i}{\tilde{\sigma}_i} \right);\\
    \omega \left(1-\Phi\left(\frac{t_i+\Delta_i-\tilde{\mu}_i}{\tilde{\sigma}_i}\right)\right) &={\mathscr P}'(\Delta_i),
\end{align*}
if the optimum corresponds to a stationary point. 
\iffalse
First we fix $t_i$ and try to determine $\Delta_i(t_i)$. Observe that the left-hand side of \eqref{eq:FP} decreases in $\Delta_i$, and goes to $0$ as $\Delta_i\to\infty$, with its maximal value being
\[\Delta_i^+(t_i):=  \omega\left(1-\Phi\left(\frac{t_i-\tilde{\mu}_i}{\tilde{\sigma}_i} \right)\right).\]
It is readily checked that this means that there is a solution if 
\[\omega \geq \Phi\left(\frac{t_i-\tilde{\mu}_i}{\tilde{\sigma}_i} \right),\]
this solution being
\begin{align*}
    \Delta_i(t_i) = 
    \tilde{\sigma}_i \Phi^{-1}
    \left(
    1 - \frac{1-\omega}{\omega}
    \Phi\left(\frac{t_i-\tilde{\mu}_i}{\tilde{\sigma}_i} \right)
    \right) + \tilde{\mu}_i - t_i.
\end{align*}
Now, again considering the domain in which the optimum corresponds to a stationary point of the objective function, by considering the partial derivative of the objective function with respect to $\Delta_i$, 
we can determine $t_i$ as
the root of
\[\omega \left(1-\Phi_i\left(\frac{t_i+\Delta_i(t_i)-\tilde{\mu}_i}{\tilde{\sigma}_i}\right)\right) -f'(\Delta_i(t_i))=0.\]
\fi
To get a better intuition for these equations, consider again the specific example of ${\mathscr P}(\Delta) = \alpha \Delta$ for some $\alpha\leqslant \min\{\omega,1-\omega\}$.
We find that the window is
\[\left(\tilde\mu_i +\tilde\sigma_i\Phi^{-1}\left(\frac{\alpha}{1-\omega}\right),
\tilde\mu_i +\tilde\sigma_i\Phi^{-1}\left(1-\frac{\alpha}{\omega}\right)
\right);\]
evidently, if the left boundary of the interval happens to drop below 0, it is to be replaced by~$0$.
If $\omega\not=\frac{1}{2}$, the window is asymmetric around $\tilde\mu_i.$ Indeed, as is readily checked, the midpoint of the interval lies at 
\[\tilde\mu_i +\frac{\tilde\sigma_i}{2}\left(\Phi^{-1}\left(1-\frac{\alpha}{\omega}\right)-\Phi^{-1}\left(1-\frac{\alpha}{1-\omega}\right)\right).\]
This midpoint is larger than $\tilde\mu_i$ if $\omega<\frac{1}{2}$ and smaller than $\tilde\mu_i$ if $\omega>\frac{1}{2}$, in line with the weights assigned to the deliverer being late and early, respectively. Also observe that the width of the window is decreasing in $\alpha$: the more the width is penalized, the more narrow the optimal window is. In the special case that the service times are all $N(\mu,\sigma^2)$, then the window is of the form
\[\left(i\mu +\sigma\sqrt{i}\,\Phi^{-1}\left(\frac{\alpha}{1-\omega}\right),
i\mu +\sigma\sqrt{i}\,\Phi^{-1}\left(1-\frac{\alpha}{\omega}\right)
\right)\]
for $i\in\{1,\ldots,n\}$; again, if the left boundary is smaller than 0, it is replaced by $0$. We conclude that in this homogeneous scenario the windows are intervals around $i\mu $ (not necessarily symmetric) with a width that is proportional to $\sqrt{i}$. 

% Actually, in case $f(\Delta) = \alpha \Delta$, it should be noted that $\omega = 1/2$ is the \textit{only} value of $\omega \in (0,1)$ for which a solution to the above
% set of equations can be found for all $\alpha$. That is,
% since the lhs of both equations is the same,
% we observe that
% \begin{align*}
%     (1-\omega)\Phi\left(
%     \frac{t_i - \tilde{\mu}}{\tilde{\sigma}}
%     \right) = \alpha,
% \end{align*}
% such that $\alpha \leq 1 - \omega$ should
% hold, yielding 
% \begin{align*}
%     t_i = \tilde{\mu} + \tilde{\sigma}
%     \Phi^{-1}\left(\frac{\alpha}{1-\omega} \right).
% \end{align*}
% Substituting this into the second
% equation, we find that a corresponding
% $\Delta_i$ exists only if $0 \leq 1 - \alpha/\omega \leq 1$, such that $\alpha \leq \omega$. Together with the 
% fact that $\alpha \leq 1 - \omega$, we 
% obtain that $\omega = 1/2$ is the only
% value of $\omega$ that yields a solution
% for all $\alpha$.

% \begin{example} \em 
%  \textcolor{red}{ Now we will consider the case with $B_i\sim {\rm Exp}(\lambda_i)$, sum $S_i$ follows hypoexponential distribution. 
%   \[
% F_{S_i}(x) = 1 - \sum_{j=1}^i \left( \frac{\prod_{k=1, k \neq j}^i \lambda_k}{\prod_{k=1}^i (\lambda_k - \lambda_j)} \right) e^{-\lambda_j x}
% \]}
% \end{example}

% \begin{example} \em 
%     \textcolor{red}{ Approximate (or find) $S_i$ with a Weibull distribution, can find a fit for mean and variance. Consider $W_i \sim {\rm W} (k, \lambda)$
% \begin{itemize}
%     \item The mean of the Weibull distribution $W$ is given by:
%     \[
%     \mathbb{E}[W] = \lambda \Gamma\left(1 + \frac{1}{k}\right),
%     \]
%     where $\Gamma$ is the Gamma function.
%     \item The variance of $W$ is:
%     \[
%     \text{Var}(W) = \lambda^2 \left( \Gamma\left(1 + \frac{2}{k}\right) - \left(\Gamma\left(1 + \frac{1}{k}\right)\right)^2 \right).
%     \]
% \end{itemize}
% We want these to match the mean and variance of $S_i$, which are $\tilde{\mu}$ and $\tilde{\sigma}^2$, respectively.
% So, we set:
% \[
% \lambda \Gamma\left(1 + \frac{1}{k}\right) = \tilde{\mu},
% \]
% \[
% \lambda^2 \left( \Gamma\left(1 + \frac{2}{k}\right) - \left(\Gamma\left(1 + \frac{1}{k}\right)\right)^2 \right) = \tilde{\sigma}^2.
% \]
% }
% \end{example}

% \begin{example} \em 
% \textcolor{red}{Let $B_i \equiv T_i(X(t)) + A_i$, where $A_i$ is a random variable that encodes the drop on/off time, and $T_i$ a random variable that models the travel time from location $i-1$ to location $i$, which is dependent on the state of a Markov process $X(t)$ encoding network conditions.}
% \end{example}

Whereas we find an explicit characterization of
the window in case $\mathscr{P}(\Delta) = \alpha \Delta$,
other penalty functions typically require numerical
optimization. Figure~\ref{fig: normal_wos} displays the `centered
windows' $[t_i - \mu_i, t_i + \Delta_i - \mu_i]$ 
for
various parameter values {in case ${\mathscr P}(\Delta) = (\alpha/\beta) \Delta^\beta$}. 
\begin{itemize}
    \item[$\circ$] 
It can be observed that the impact 
of $\omega$ aligns with the observations above:
$\omega = \frac{1}{2}$ yields a symmetric window,
but when $\omega < \frac{1}{2}$ (resp.\ $\omega > \frac{1}{2}$)
the penalty for early (resp.\ late) arrivals becomes dominant, 
% over penalties
% for being too early (resp.\ late), 
and the optimal \(t_i\) shifts to an earlier 
(resp.\ later) time. 
We also observe symmetry
in the windows of $\omega$ and $1-\omega$, in that
the  centered window of $1-\omega$ is the mirrored
(in the time axis value of 0) centered window of $\omega$.
 \item[$\circ$] 
As \( \alpha \) scales the penalty linearly, higher values of $\alpha$
result in tighter time windows. 
% Simultaneously, \( t_i \) shifts closer to the mean \( \mu_i \) as \( \alpha \) increases, reflecting the system's effort to centralize around the mean and minimize penalties symmetrically. 
The impact of $\beta$ is less trivial, as it is dependent on the value
of $\Delta$: 
%Which is noticeable for larger \( \beta \), as 
the penalty for \( \Delta > 1 \) grows steeply with higher \( \beta \), 
% further constraining \( \Delta_i \) at small \( \alpha \). Interestingly, for \( \alpha > 0.25 \), 
% but for $\Delta < 1$ the behavior reverses: \( \Delta_i \) increases with higher \( \beta \), as the penalty curve 
but flattens for \( \Delta < 1 \).
% this enables more flexibility for larger deviations. 
Therefore, the order of the \( \Delta_i \) values with respect to \( \beta \) undergoes a transition, in that
% in Figure~\ref{fig: normal_wos}, 
% \( \Delta_i \) is essentially inversely proportional to \( \beta \)
% for \( \alpha = 0.1 \), 
% but becomes  proportional to \( \beta \)
% for the other values of $\alpha$. 
% Indeed, 
for \( \alpha = 0.1 \) the smallest value of $\beta$ yields
the largest time-windows width, whereas
for $\alpha = 0.25, 0.5$ the smallest value of $\beta$ yields the smallest time-window width.
% \footnote{MM: this last sentence I don't get.}
\end{itemize}

% Include numerical examples normal
% distribution:
% \begin{itemize}
%     \item 9 plots with normal distribution, describe effect of alpha, beta, omega
%     \item one different plot in which the lines intersect 
% \end{itemize}

\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{Figures/ti_windowi_matrix_1025.png}
    \caption{{WOS time windows for normally distributed travel times with } parameters $\mu_i = 10$ and $\sigma_i = 2.5$. The three rows correspond to $\omega=0.25, 0.5, 0.75$, respectively, and the three columns to $\alpha = 0.1, 0.25, 0.5$, respectively. }
    \label{fig: normal_wos}
\end{figure}

It is interesting to note that the symmetry of the windows around $\tilde{\mu}_i$ that is observed for $\omega = \frac{1}{2}$ holds more generally: it is true for any penalty function $\mathscr{P}(\cdot)$
satisfying the conditions of Theorem~\ref{THM1} and any service time
distribution that is symmetric in some $\mu_i$. 
As it turns out, the same conditions are also sufficient
for the mirrored windows of $\omega$ and $1-\omega$. The following lemma makes these claims formal. 

\begin{lemma}\label{lem: symmetry}
Let ${\mathscr P}(\cdot)$ be strictly convex, 
$g(\Delta):={\mathscr P}'(\Delta)$ have a continuous inverse, 
and the probability density function of $S_i$ be symmetric in $\mu_i \in \mathbb{R}_{+}$.
Then, if $[t(\omega'), t(\omega') + \Delta]$ is the
optimal window for $\omega = \omega'$, 
$[t(1-\omega'), t(1-\omega') + \Delta]$ is the
optimal window for $\omega = 1-\omega'$, where $t(1-\omega')$ is such that
\begin{align} \label{eq: omega_prime}
t(\omega') - \mu_i + \Delta = -(t(1-\omega') - \mu_i).
\end{align}
In the special case $\omega = \frac{1}{2}$, the window of client~$i$ is symmetric around
$\mu_i$.
\end{lemma}

{\it Proof.}
By Theorem~\ref{THM1}, $(t(\omega'), \Delta)$ is the unique
solution to \eqref{FOC1} and \eqref{FOC2}
for $\omega = \omega'$, such that
\begin{align} \label{eq: opt_omega_prime}
    (1-\omega') F_i(t(\omega')) = \omega'\left(1-F_i(t(\omega') + \Delta )\right) = \mathscr{P}'(\Delta).
\end{align}
Now, the symmetry of the probability density function of $S_i$ in $\mu_i$
yields that $F_i(\mu_i - x) = 1-F_i(\mu_i + x)$, 
from which we obtain
\begin{align*}
    F_i(t(1-\omega'))
    =F_i\left(\mu_i - (\mu_i-(1-\omega'))\right)
    =1-F_i(-t(1-\omega') + 2\mu_i)
    =1-F_i(t(\omega') + \Delta)
\end{align*}
and
\begin{align*}
    1-F_i(t(1\!-\!\omega') + \Delta)
    =1-F_i(\mu_i + t(1\!-\!\omega') + \Delta - \mu_i)
    =F_i(2\mu_i - t(1\!-\!\omega') - \Delta)
    =F_i(t(\omega')).
\end{align*}
Hence, \eqref{eq: opt_omega_prime} yields that
both $\omega' F_i(t(1-\omega'))$ and
$(1-\omega')\left(1-F_i(t(1-\omega') + \Delta)\right)$
equal $\mathscr{P}'(\Delta)$, making
$[t(1-\omega'), t(1-\omega') + \Delta]$ the optimal
window for $\omega = 1-\omega'$. Note that
for $\omega = \frac{1}{2}$, \eqref{eq: omega_prime} implies
\begin{align*}
    |t(1/2) + \Delta_i - \mu_i|
    = |t(1/2) - \mu_i|,
\end{align*}
as desired.
\hfill$\Box$

\subsection{WOS under general convolutions}\label{subsec:WOSgen}
If a closed-form expression for the distribution function $F_i: \mathbb{R}_{+} \to [0,1]$ of $S_i$ is not available, it can be evaluated numerically by iteratively convolving discretized versions of the travel-time distributions. While this is in principle also possible when the travel times are dependent, in this section we focus on the case that they are independent. 
The idea is to simply discretize the continuous random variables $B_i$, $i = 1,\dots,n$, over a grid from $\mu_i-b_i$ to $\mu_i+b_i$,
for some $b_i \in \mathbb{R}_+$, using
a step size of $\varepsilon$. Then the arrival time distributions at the different client locations follow from a sequential numerical convolution
of these discrete distributions. Concretely, 
the arrival time distribution of client~$j$
follows from convolving the arrival time distribution
of client $j-1$ and the distribution $B_j$.
In all experiments below,
we have used $b_i = 4\sigma_i$ and a step size of $\varepsilon = 10^{-3}$, with $\sigma_i$ the standard deviation of $B_i$.

% Briefly summarized, 
% let $t_{l,i}, t_{u,i} \in \mathbb{R}$
% be such that
% $\mathbb{P}(t_{l,i} \leq B_i \leq t_{u,i}) \geq 1-\gamma$ for
% some small $\gamma > 0$. Then, 
% the distribution of $B_i - \mu_i$,
% where $\mu_i$ is the mean of $B_i$,
% can be captured
% in a list of $n$ pairs $(t_j, p_j)$,
% where $t_j = -t_{l,i} + j\frac{n}{t_{u,i} + t_{l,i}}$ is value in some range
% $[-t_{l,i}, t_{u,i}]$ and $p_j$
% Let $t_l, t_u \in \mathbb{R}$ be such that
% $\mathbb{P}(-t_l \leq B_i - \mu_i \leq t_u) \geq 1-\gamma$ for all $i = 1,\dots,n$ and some
% small $\gamma > 0$, where $\mu_i$ is
% the mean of $B_i$.
% For a discretization parameter $n$,
% the discretized
% distribution of $B_i - \mu_i$ can be captured
% in a list of $n$ pairs $(t_j, p_j)$,
% where $t_j = -t_l + \frac{j}{t_u + t_l}$
% and $p_j = \mathb{P}()$



% times, the distribution of $S_i$ which is needed
% to compute $(t_i, \Delta_i)$ from 
% \eqref{FOC1} and \eqref{FOC2}



% \begin{figure}
%     \centering
%     \includegraphics[width=0.75\linewidth]{Figures/upd/ti_windowi_mu10lognormal.pdf}
%     \caption{logormal distribution, parameters $\mu_i = 10.0$ and $\sigma_i = 2.5$.}
%     \label{fig:exp1_logn}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.75\linewidth]{Figures/upd/ti_windowi_mu10weibull.pdf}
%     \caption{Weibull distribution, parameters $\mu_i = 10.0$ and $\sigma_i = 2.5$.}
%     \label{fig:exp1_weib}
% \end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figures/upd/subplots_comparison_smallnormal_vs_weibull_vs_lognormal.pdf}
    \caption{
    {WOS time windows using numerical convolutions; we use the same mean and standard deviation $\mu_i = 10$ and $\sigma_i = 2.5$ for all distribution functions.}} %All three methods $\mu_i = 10.0$ and $\sigma_i = 2.5$.}
    \label{fig:exp1_v1}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{Figures/upd/differences_comparison_new.pdf}
    \caption{Difference of time windows for Weibull and Lognormal distribution, relative to time windows for normal distribution.
    \Rene{A legend is missing explaining the colours}}
    \label{fig:normal_approx_difference}
\end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{Figures/upd/Time_Dynamic.pdf}
%     \caption{Run-time for updated dynamic procedure}
%     \label{fig:enter-label}
% \end{figure}

Figure~\ref{fig:exp1_v1} illustrates the time windows resulting from the convolution method across three different distributions: normal, Weibull, and Lognormal. As before, these time windows have been `centered', meaning that the mean $\mu_i$ has been subtracted for each client $i$. {The mean and standard deviation of the service times are 10 and 2.5, respectively, for all clients and distributions. With these parameters, the normal and Weibull distributions exhibit similar, symmetric shapes, resulting in nearly identical time windows.}
%Throughout these experiments, we maintained constant means and variances for all clients and for all three distributions. For the parameters used, the densities of the normal and Weibull distributions exhibit similar, symmetric shapes, causing their time windows to be nearly identical. 
In contrast, the density of the Lognormal distribution is significantly skewed, leading to {somewhat different} %distinct 
time windows. Specifically, for $\omega = 0.5$, the Lognormal time windows are not symmetric around zero.
It is worth noting that, for all the settings shown in Figure~\ref{fig:exp1_v1}, the endpoints of the time windows under the Lognormal distribution occur earlier than those under the Weibull and normal distributions. This effect arises because the Lognormal distribution has a greater probability mass to the left of the mean, compared to the other two distributions.

Figure~\ref{fig:exp1_v1} considers the case of $n = 6$ customers. 
{Although computations remain feasible for larger values of $n$, the numerical evaluation of convolutions becomes increasingly demanding, as the number of bins required grows with the number of clients.} %It is noted that it is challenging to perform the computations for large values $n$, as it requires the numerical evaluation of the convolution, where the number of bins that are to be used grows with the number of clients.
One potential speed-up, at the cost of a small loss
in accuracy, is to bound the total number of bins that may arise after a convolution step by changing the bin-size and allowing for larger bins, i.e., by increasing $\varepsilon$, thereby re-distributing the weights of the bins (e.g., 
using interpolation). 

A more convenient solution to cope with the computational burden, however, is to approximate, for sufficiently high client indices $i$, the $S_i$ by their normally distributed counterparts. 
This approximation is motivated by the central limit theorem, noting that $S_i$ is the sum of random variables. 
In particular, for any client $i\geqslant i_0$, 
we set $S_i \sim N({\mu}_i, {\sigma}_i^2)$, where ${\mu}_i$
and ${\sigma}_i^2$ are the mean and 
variance of the true arrival time distribution,
respectively; in the literature often $i_0=15$ is being used. The idea is that the use of this normal approximation significantly reduces computational costs
while maintaining reasonable accuracy.

The accuracy of the normal approximation is illustrated in Figure~\ref{fig:normal_approx_difference} for cases in which the $B_i$ follow a Weibull or Lognormal distribution.
The figure shows a typical example of the differences in the resulting time windows.
\Rene{What is being plotted? Is this the difference between start and end times? This should be clearly stated.}
A comparison in the value of the objective function (based on $R=10^9$ simulation runs)
for the same distributions is given in Table~\ref{tab:performance_runtime_2}.
Specifically, for both distributions, time windows are computed using (a)~the normal approximation, (b)~the convolution method, and (c)~a combined approach applying convolution to the first 15 clients and the normal approximation to the remainder.
For these sets of time windows, we evaluate the value of the objective function $G_n(\boldsymbol{t}, \boldsymbol{\Delta})$ using Monte Carlo simulation, that is, by $R$ times sampling the $n$ 
random variables $B_i$, evaluating for those sampled $B_i$ the value of the objective function, and taking their average (that is, add the $R$ realized values of the cost function and divide by $R$). We also calculated the percentage error of the normal approximation relative to the (exact) convolution-based value, indicated by $\Delta_{\rm app}^i$, and the percentage error of the combined method relative to the (exact) convolution-based value, denoted by $\Delta_{\rm com}^i$; here $i\in\{{\rm W},{\rm LN}\}$, where W stands for Weibull and LN for Lognormal. 
As can be observed from Table~\ref{tab:performance_runtime_2},
for both $B_i$ having a Lognormal and a Weibull distribution,
there are virtually negligible differences between the output obtained via the three methods. As the convolution method is considerably more time consuming than the normal approximation, this table suggests to use the normal approximation. 

In Table~\ref{tab:performance_runtime_2}, the clients' travel times are assumed i.i.d. To stress-test the normal approximation, Table~\ref{tab:non_iid_variance_sin} considers a setting where the variances of the $B_i$'s vary with the client index, using $\sigma_i = 2.5 + 1.5 \sin\left(\frac{2\pi i}{10}\right)$. Even in this heterogeneous setting, the normal approximation remains highly accurate. The run times are omitted because they are virtually identical to those reported in Table~\ref{tab:performance_runtime_2}.

In the above experiments, we picked specific values for the parameters of the underlying model. The last experiment of this section aims to show that the above conclusions carry over to a broad range of such parameters. 
Figure~\ref{fig:normal_approx_difference} describes the effect of stronger client heterogeneity,
for three values of the number of clients $n$ and estimates based on simulation runs $R = 10^7$. In each scenario, the values of $\omega, \alpha$, and $\beta$ are selected uniformly at random from predefined sets (given in the caption of the figure).
Likewise, each travel-time distribution is
randomly selected to be normal, lognormal or Weibull, with mean $\mu$
selected, again uniformly at random, from predefined sets as well (also given in the caption of the figure); the variance $\sigma^2$ is kept at 2.5 for each travel time. 
For each experiment, we compute the objective function, with (a)~the windows based on the normal approximation and  (b)~the windows based on the convolution method, and then we compute their percentage difference,
so as to assess the accuracy of the normal approximation. These percentage differences are shown in the boxplot of Figure~\ref{fig:normal_approx_difference}. 
The main conclusion from the boxplot is that the normal approximation is highly accurate across the broad range of heterogeneous scenarios that were studied.
%This trade-off is crucial, as the growing number of operations per client makes continued convolution impractical for large-scale simulations.
% Each convolution operation involves a
% summation over all bin-pairs of the two
% considered distributions, such that the
% complexity in each step is a product
% of the number of bins of the two distributions.
% Since the sequential convolutions for each additional client in the system, the computational burden increases significantly, making direct convolution infeasible for large $n$. 

%\begin{landscape} % Rotate the table for better fit
\iffalse
\begin{table}[h]
    \centering
    \resizebox{\textwidth}{!}{ % Auto-resize table to fit page width
    \begin{tabular}{lcccccc|cccccc}
        \toprule
        \multicolumn{1}{c}{\textbf{B$_i$’s iid, $\alpha = 0.05$, $\beta = 1.1$}} & \multicolumn{6}{c}{\textbf{Performance (Separate values of three components of objective function)}} & \multicolumn{6}{c}{\textbf{Runtime to evaluate $t_i$ and $\delta_i$ (s)}} \\
        \cmidrule(lr){2-7} \cmidrule(lr){8-13}
        & 20 & 40 & 60 & 80 & 100 & 120 & 20 & 40 & 60 & 80 & 100 & 120 \\
        \midrule
        \textbf{Approxn (WL)} & 31.1498 & 88.7669 & 164.1973 & 254.0456 & 357.6421 & 472.0459 & 0.0691 & 0.1108 & 0.1826 & 0.2490 & 0.4273 & 0.3775 \\
        \textbf{Conv dynamic (Weibull)} & 31.1350 & 88.6608 & 164.1283 & 254.3399 & 357.4375 & 472.1881 & 13.6808 & 49.2947 & 108.2617 & 187.1384 & 284.9909 & 421.2618 \\
        \textbf{Conv (15) + Approxn (WL)} & 31.1407=5.0612+5.2488+20.8307 & 88.6464=14.9244+15.0520+58.6701 & 164.1175=27.8938+28.2416+107.9821 & 254.4266=43.7678+43.9983+166.6605 & 357.0610=61.6843+61.9045+233.4722 & 472.0893=82.0033+82.5074+307.5786 & 11.0445 & 11.3923 & 11.5012 & 11.8901 & 12.2023 & 12.6315 \\
        \textbf{Conv dynamic (Logn)} & 31.1167 & 88.6342 & 164.0607 & 254.3033 & 357.3690 & 472.0730 & 15.0520 & 52.8340 & 115.6297 & 200.0013 & 300.3289 & 416.8669 \\
        \textbf{Conv (15) + Appn (higher)} & 31.1235 & 88.5935 & 164.1492 & 254.2022 & 357.6291 & 472.3499 & 8.9236 & 8.8983 & 8.8268 & 8.8868 & 8.9302 & 9.1041 \\
        \bottomrule
    \end{tabular}
    }
    \caption{Performance and Runtime Comparisons}
    \label{tab:performance_runtime}
\end{table}
%\end{landscape}
\fi

%\begin{landscape} % Rotate the table for better fit
%\blue{\[ \Delta_A^B= \frac{B(A)-conv(A)}{conv(A)}\]}

{\small
\begin{table}
    \centering
   % \resizebox{\textwidth}{!}
    { % Auto-resize table to fit page width
    \begin{tabular}{lrrrrr}
        \toprule
        \multicolumn{1}{c}{\textbf{}} & \multicolumn{5}{c}{\textit{Objective function}} \\ % & \multicolumn{6}{c}{\textbf{Runtime (s)}} \\
        \cmidrule(lr){2-6} %\cmidrule(lr){8-13}
        number of clients $n$& 20 & 40 & 60 & 80 & 100  \\ %& 20 & 40 & 60 & 80 & 100  \\
         \midrule
        {Weibull -- convolution} & 54.4714 & 155.8506 & 288.7246 & 447.1245 & 627.7793  \\
        {Runtime (s)} & 11.4558 & 39.1289 & 89.0035 & 138.9098 & 215.2231  \\
        \midrule
        {Weibull -- normal approximation} & 54.3346 & 155.7097 & 288.5674 & 447.0486 & 627.6036  \\
        {Runtime (s)}& 0.0555 & 0.0650 & 0.1048 & 0.1442 & 0.1566  \\
        \midrule
        {Weibull -- combined} & 54.4300 & 155.7639 & 288.3891 & 447.0403 & 627.6280  \\
        {Runtime (s)} & 6.1227 & 6.2407 & 6.2304 & 6.6787 & 6.6930  \\
         \midrule
        {Lognormal -- convolution} & 54.2104 & 155.4583 & 288.2273 & 446.6121 & 627.2115   \\
        {Runtime (s)} & 10.1897 & 37.0350 & 80.2342 & 136.5655 & 207.5953   \\
        \midrule
        {Lognormal -- normal approximation} & 54.4198& 155.7562& 288.4493& 446.4572& 627.8023  \\
        {Runtime (s)} &0.0560 & 0.0561 &0.0818& 0.1140& 0.1392   \\
        \midrule
        {Lognormal -- combined} & 54.2375 & 155.5400 & 288.4854 & 447.0526 & 626.8255   \\
        {Runtime (s)} & 6.8032 & 6.0899 & 6.1362 & 6.4429 & 6.4074   \\
        \midrule 
       \textbf{$\Delta_{\rm app}^{\rm W}$}  &-0.25	&-0.09	&-0.05	&-0.02	&-0.003	   \\
       \textbf{$\Delta_{\rm com}^{\rm W}$} &-0.08 &-0.06 &-0.12 &-0.02 &-0.02   \\
        \textbf{$\Delta_{\rm app}^{\rm LN}$} & 0.38& 0.19&0.08 & -0.03& 0.09  \\
        \textbf{$\Delta_{\rm com}^{\rm LN}$} &0.04 &0.05 & 0.09 & 0.10 &-0.06    \\
        \bottomrule
    \end{tabular}}
    \caption{Accuracy and runtime comparisons, for $B_i$\,s i.i.d., $\alpha = 0.1$, $\beta = 1.5$.
    \Rene{Change the layout of this table? It claims to show the objective function, but actually also shows runtimes. The $\Delta$ at the end is also not ideal (but may be the best??)}}
    \label{tab:performance_runtime_2}
\end{table}}

% \begin{table}[h]
%     \centering
%     \resizebox{\textwidth}{!}{ % Auto-resize table to fit page width
%     \begin{tabular}{lccccc|ccccc}
%         \toprule
%         \multicolumn{1}{c}{\textbf{B$_i$’s not-iid (sin function), $\alpha = 0.1$, $\beta = 1.5$}} & \multicolumn{5}{c}{\textbf{Performance}} & \multicolumn{5}{c}{\textbf{Runtime (s)}} \\
%         \cmidrule(lr){2-6} \cmidrule(lr){7-11}
%         & 20 & 40 & 60 & 80 & 100 & 20 & 40 & 60 & 80 & 100 \\
%         \midrule
%         \textbf{Approx} & 54.4165 & 155.7841 & 288.4311 & 446.5751 & 627.9859 & 0.0674 & 0.1273 & 0.0965 & 0.1240 & 0.3284 \\
%         \textbf{Conv dynamic (Weibull)} & 54.4050 & 155.8021 & 288.5927 & 447.0367 & 627.6692 & 11.5521 & 42.4204 & 85.4683 & 150.5094 & 246.4169 \\
%         \textbf{Conv (15) + Exact (higher)} & 54.3825 & 155.7436 & 288.5430 & 447.2644 & 627.8788 & 6.5616 & 6.6521 & 6.7196 & 6.6203 & 6.5074 \\
%         \midrule
%         \textbf{Approxn (Logn)} & 54.4482 &155.6408 & 288.5572 &  446.7779& 627.4021& 0.0628 &  0.1260 &0.1541 & 0.1242 &0.2788\\
%         \textbf{Conv dynamic (Lognormal)} & 54.2835 & 155.5883 & 288.3876 & 446.7102 & 627.3482 & 11.2453 & 39.6692 & 84.9683 & 158.9222 & 221.7947 \\
%         \textbf{Conv (15) + Exact (higher)} & 54.3101 & 155.7222 & 288.6199 & 446.9768 & 627.0657 & 7.4232 & 7.3675 & 6.9630 & 8.0491 & 8.2032 \\
%         \bottomrule
%     \end{tabular}
%     }
%     \caption{Performance and Runtime Comparisons for B$_i$’s not-iid (sin function) $ \mu_{new} = \mu + 5 * (np.\sin((i/n)*2*np.\pi) + 1) / 2 $}
%     \label{tab:performance_runtime_notiid}
% \end{table}

{\small
\begin{table}[htbp]
\centering
\caption{Accuracy comparisons, for $B_i$\,s non-i.i.d., $\alpha = 0.1$, $\beta = 1.5$.\Rene{Write more concrete caption?}}
%\resizebox{\textwidth}{!}
{%
\begin{tabular}{lccccc}
\toprule
 & \multicolumn{5}{c}{\it Objective function} \\ %& \multicolumn{5}{c}{Runtime (s)} \\
\cmidrule(lr){2-5}% \cmidrule(lr){7-11}
number of clients $n$ & 20 & 40 & 60 & 80 & 100 \\%& 20 & 40 & 60 & 80 & 100 \\
\midrule
Weibull -- normal approximation                & 40.5520 & 117.6964 & 219.1714 & 340.5374 & 479.4331 \\
Weibull -- convolution     & 40.6738 & 117.8401 & 219.3660 & 340.7553 & 479.2350 \\
Weibull -- combined  & 40.6108 & 117.5708 & 219.0133 & 340.5200 & 478.4872 \\
\midrule 
Lognormal -- normal approximation                 & 40.5922 & 117.6391 & 219.1380 & 340.7982 & 478.9577 \\ 
Lognormal -- convolution   & 40.5212 & 117.5882 & 219.0586 & 340.4068 & 478.8196 \\
Lognormal -- combined  & 40.5094 & 117.5752 & 219.1287 & 340.6473 & 478.5470  \\
\bottomrule
\end{tabular}%
}
\label{tab:non_iid_variance_sin}
\end{table}}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{Figures/upd/box20.png}
%     \caption{for 20 and 40 clients}
%     \label{fig:enter-label}
% \end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.775\linewidth]{Figures/upd/boxplot_whisk595.png}
     \caption{Boxplot assessing accuracy of the normal approximation over a broad range of heterogeneous scenarios. The hinges of the box correspond to the 25- and 75-percentiles, the whiskers to the 5- and 95-percentiles \Rene{Is this correct? Not very common in boxplots}. The predefined parameter sets used in experiments are: $\omega\in \{0.25, 0.5, 0.75\}$, $\alpha\in\{0.01, 0.05, 0.1, 0.15\}$,   $\beta\in\{1.1, 1.2, 1.3, 1.4, 1.5\} $, $\mu\in\{10, 12, 15\}$.}
    \label{fig:boxplot_errors}
\end{figure}

% Potential future numerical examples:
% \begin{itemize}
%     \item bimodal, can be explained, non-parallel lines. Small p vs big p
% \item Most interesting: compare with case we don't have p's, make sure mean of the service times is the same. Then we see the impact of correlation 
% \end{itemize}
